Fuzz on the Beach: Fuzzing Solana Smart Contracts

Solana has quickly emerged as a popular platform for building decentralized applications (DApps), such as marketplaces for non-fungible tokens (NFTs). A key reason for its success are Solana's low transaction fees and high performance, which is achieved in part due to its stateless programming model. Although the literature features extensive tooling support for smart contract security, current solutions are largely tailored for the Ethereum Virtual Machine. Unfortunately, the very stateless nature of Solana's execution environment introduces novel attack patterns specific to Solana requiring a rethinking for building vulnerability analysis methods. In this paper, we address this gap and propose FuzzDelSol, the first binary-only coverage-guided fuzzing architecture for Solana smart contracts. FuzzDelSol faithfully models runtime specifics such as smart contract interactions. Moreover, since source code is not available for the large majority of Solana contracts, FuzzDelSol operates on the contract's binary code. Hence, due to the lack of semantic information, we carefully extracted low-level program and state information to develop a diverse set of bug oracles covering all major bug classes in Solana. Our extensive evaluation on 6049 smart contracts shows that FuzzDelSol's bug oracles find bugs with a high precision and recall. To the best of our knowledge, this is the largest evaluation of the security landscape on the Solana mainnet.

==> acmart-preload-hook.tex <==
\PassOptionsToPackage{dvipsnames,svgnames,x11names}{xcolor}


==> only-text_rem.tex <==
%!TEX

\makeatletter

\onecolumn
{\centering\Huge *** TODO *** TODO *** TODO *** TODO ***\par}
% \raggedright
\pretolerance=10000
% \tolerance=1
\emergencystretch=\textwidth
\hyphenpenalty=10000
\exhyphenpenalty=10000
% \hbadness=10000
\RenewDocumentEnvironment{table}{+b}{}{}
\RenewDocumentEnvironment{table*}{+b}{}{}
\RenewDocumentEnvironment{figure}{+b}{}{}
\RenewDocumentEnvironment{figure*}{+b}{}{}
\AddToHook{cmd/section/before}{\clearpage}
\AddToHook{cmd/subsection/before}{\clearpage}
\renewcommand{\maketitle}{{\par\centering\Large\@title\par}}
\renewcommand{\printbibliography}{\par Bibliography.\par}
\renewcommand{\cite}[1]{\unskip}
\renewcommand{\Cref}[1]{Figure 0\xspace}
\renewcommand{\textsc}[1]{#1}

\RenewDocumentEnvironment{abstract}{}{\section*{Abstract}}{}

\pagestyle{empty}

\makeatother


==> sections/apx-addresses_remove.tex <==
%!TEX root = ../main.tex

\section{Program IDs}
\label{apx-addresses}

We provide the full program IDs for the programs from~\Cref{tbl:eval_bugs}.
We analyzed the programs and \tool's reports in depth during our bug finding experiment. (\Cref{sec:eval_bugs})

\begin{table}[h]
  \centering
  \begin{tabular}{@{}c|c@{}}
    \toprule
    Abbreviation & Full Program ID \\
    \midrule
    \texttt{3nJ2...5erP} & \texttt{3nJ2MWbnS3bW8rnWhejAgnLQTyiqoA5fMq5Z7jRv5erP} \\
    \texttt{3od3...jnsW} & \texttt{3od3X7QN84FTonkyXbQiT1ydxcT9P1jBcA9mbgD3jnsW} \\
    \texttt{3Vtj...4q8v} & \texttt{3VtjHnDuDD1QreJiYNziDsdkeALMT6b2F9j3AXdL4q8v} \\
    \texttt{3w57...obPW} & \texttt{3w57iMhv5Zk5VDuTe5dspm2FzE9zQhscCb9CZpAKobPW} \\
    \texttt{4hPk...JP5N} & \texttt{4hPkNV2WsgPW1wHHcQebvV7GLyLgdDDLEx3Pu6LzJP5N} \\
    \texttt{4M2f...jStx} & \texttt{4M2fancicHbUtMLcMNmbi97YngFoqBcnFk5D31JjjStx} \\
    \texttt{6Lan...szqi} & \texttt{6LanqAFCbucXWSG35ssij4kFDTWJ25BY7d6hbR2szqi} \\
    \texttt{7FWE...9p7p} & \texttt{7FWEcVG1YRW7evGR3bXgu47ge8m6Je7BQuvTzMbn9p7p} \\
    \texttt{9a5d...jZP9} & \texttt{9a5dihgNgBhWnjmRDJ8rUy4ihetvgMmjaPk7NGdsjZP9} \\
    \texttt{9tSW...11yy} & \texttt{9tSWsKwtDL6YseLuh1haGFJk312uu9HGyrnVa5XH11yy} \\
    \texttt{GQ6q...1u6K} & \texttt{GQ6qchUsofiK7rzeFg5jbvpHcJ7pNnfL4yfwaYrB1u6K} \\
    \texttt{9WoL...849B} & \texttt{9WoLnfjLKk1EBtkABhe3vcA8CLogsbs3XBoddn8h849B} \\
    \texttt{H5rp...nPSG} & \texttt{H5rpfCD6hLFCPCfxxqjGg94Gqoigqfk7afhqGLu1nPSG} \\
    \bottomrule
  \end{tabular}
  \caption{Program IDs and abbreviations from~\Cref{tbl:eval_bugs}.}%
  \label{tbl:full-addresses}
\end{table}


\section{Oracle algorithms}\label{apx-oracle-algorithms}

In the following, we provide a detailed explanation of the \emph{missing owner check oracle}, \emph{arbitrary CPI oracle}, \emph{missing key check oracle} and \emph{integer bugs oracle}.

\subsection{Missing Owner Check Oracle}
\label{apx-moco}


\Cref{algorithm:missing_owner_check} details the bug-detecting process of the \emph{missing owner check oracle}.
The oracle operates as follows:
Before the program starts, the oracle initializes \emph{i)} a set $M$ in which it stores potentially malicious accounts (see Line \ref{missing_owner_check_1}) and \emph{ii)} a set of accounts $V$ that an attacker could potentially exploit using a missing owner check vulnerability (see Line \ref{missing_owner_check_2}).

At runtime of the program, the oracle checks if the program reads the data of an account $a$ which is not owned by the program, i.e., whose public key in the owner field is not equal to the program ID of the program (see Line \ref{missing_owner_check_3} and \ref{missing_owner_check_4}).
If the program does not own account $a$, the oracle marks $a$ as potentially malicious by adding it to set $M$ (see Line \ref{missing_owner_check_5}).

Moreover, the oracle checks at runtime whether the program compares account details of two account $a, b$ in registers (see Line \ref{missing_owner_check_6} to \ref{missing_owner_check_8}). 
In this comparison, if data from an account $a$ is compared to the public key of an account $b$, and $a$ is included in the set $M$ (see Line \ref{missing_owner_check_9}), the oracle marks $b$ as potentially vulnerable by adding $b$ to the set $V$ (see Line \ref{missing_owner_check_10}).
The same applies if the order of accounts in the register comparison is reversed, i.e., if the public key of account $a$ is compared with data of a account $b$ (see Line \ref{missing_owner_check_11} and \ref{missing_owner_check_12}). 
Thus, the oracle memorizes that the program has compared the data of an account potentially controlled by the attacker with the public key of another account.

The oracle signals the eBPF VM in case the program deducts lamports of an account which is contained in the set $V$, i.e., whose public key was previously compared with data of an account not owned by the program (see Line \ref{missing_owner_check_13} to \ref{missing_owner_check_17}).
The same applies when the program writes to the data field of an account contained in the set $V$ (see Line \ref{missing_owner_check_18} and \ref{missing_owner_check_19}).
This is because the oracle assumes that an owner check is missing because \emph{i)} the program compared the data of an account $a$ possibly controlled by the attacker with the public key of another account $b$ \emph{ii)} and then modified the lamports or data field of $b$.
An owner check would have already crashed the program, because the owner of the account whose data the program compared with a public key is not the program.

\begin{algorithm}
\caption{Missing Owner Check Oracle}
\label{algorithm:missing_owner_check}
\begin{algorithmic}[1]
%    \Function{MissingSignerCheckOracle}{}
        \State $M \gets \emptyset$           \label{missing_owner_check_1}
        \State $V \gets \emptyset$           \label{missing_owner_check_2}
        
        \While{program running}
            
            \If{program reads data of account $a$}                          \label{missing_owner_check_3}
                \If{$a$.owner $\neq$ program\_id}                           \label{missing_owner_check_4}
                    \State $M \gets M \cup \{a\}$                           \label{missing_owner_check_5}
                \EndIf
            \EndIf
            
            \If{program performs register comparison}                       \label{missing_owner_check_6}
                \State $a \gets \text{account in } src \text{ register}$    \label{missing_owner_check_7}
                \State $b \gets \text{account in } dst \text{ register}$    \label{missing_owner_check_8}

                \If{$a$.data \textbf{is compared with} $b$.pubkey \textbf{and} $a \in M$}       \label{missing_owner_check_9}
                    \State $V \gets V \cup \{b\}$                                               \label{missing_owner_check_10}
                \Else{ $a$.pubkey \textbf{is compared with} $b$.data \textbf{and} $b \in M$}    \label{missing_owner_check_11}
                    \State $V \gets V \cup \{a\}$                                               \label{missing_owner_check_12}
                \EndIf
            \EndIf
            
            \If{program writes to lamports field of account $a$}                \label{missing_owner_check_13}                   
                \State $l_{prev} \gets$ lamports of $a$ before write            \label{missing_owner_check_14}
                \State $l_{after} \gets$ lamports of $a$ after write            \label{missing_owner_check_15}
                \If{$a \in V$ \textbf{and}  $l_{after}$ $<$ $l_{prev}$}         \label{missing_owner_check_16}
                    \State signal VM                                            \label{missing_owner_check_17}
                \EndIf
            \EndIf
            
            \If{program writes to data of account $a$ \textbf{and} $a \in V$}   \label{missing_owner_check_18}                           
                \State signal VM                                                \label{missing_owner_check_19}
            \EndIf

        \EndWhile
%    \EndFunction
\end{algorithmic}
\end{algorithm}







\subsection{Arbitrary CPI Oracle}\label{apx-cpi}
\Cref{algorithm:arbitrary_cpi} provides a detailed explanation of the \emph{arbitrary CPI oracle}.
The oracle operates as follows:
Before starting the program, we define a malicious public key, which represents a malicious program controlled by the attacker (see Line \ref{arbitrary_cpi_line_1}).
At runtime of the program, the oracle then checks whether the program calls the functions \texttt{sol\_invoke\_signed\_rust()} or \texttt{sol\_invoke\_signed\_c()} (see Line \ref{arbitrary_cpi_line_2}). 
If this is the case, the oracle determines the public key of the called program (see Line \ref{arbitrary_cpi_line_3}). 
The oracle then checks if the public key of the program being invoked is equal to that of the previously defined malicious program (see Line \ref{arbitrary_cpi_line_4}).
This implies that an attacker is able to invoke his malicious program. 
If this is the case, the oracle signals the virtual machine (see Line \ref{arbitrary_cpi_line_5}).

\begin{algorithm}
\caption{Arbitrary CPI Oracle}
\label{algorithm:arbitrary_cpi}
\begin{algorithmic}[1]
%\Function{ArbitraryCPIOracle}{}
\State $m_{pk} \gets \text{predefined malicious public key}$                                \label{arbitrary_cpi_line_1}
\While{program is running}
    \If{program calls \texttt{sol}\_\texttt{invoke}\_\texttt{signed}\_\texttt{rust()} \textbf{or} \texttt{sol}\_\texttt{invoke}\_\texttt{signed}\_\texttt{c()}}     \label{arbitrary_cpi_line_2}
        \State $i_{pk} \gets $ public key of invoked program                             \label{arbitrary_cpi_line_3}
        \If{$i_{pk} = m_{pk}$}                                                              \label{arbitrary_cpi_line_4}
                \State signal VM                                                            \label{arbitrary_cpi_line_5}
        \EndIf
    \EndIf
\EndWhile
%\EndFunction
\end{algorithmic}
\end{algorithm}

\subsection{Missing Key Check Oracle}\label{apx-key}
\Cref{algorithm:missing_key_check} details the bug-detecting process of the \emph{missing key check oracle}.
Before the program starts, we pass two parameters to the oracle: 
First, the address of a function $f$ for which a key check is expected (see Line \ref{missing_key_check_line_1}).
Second, the public key $a_{pk}$ of an account, where the program is expected to compare the public key of an account it passes to function $f$ with the public key $a_{pk}$ before calling function $f$ (see Line \ref{missing_key_check_line_2}).
In the case of Wormhole, $f$ would represent the function \emph{load\_instruction\_at} and $a_{pk}$ would represent the public key of the \emph{KeccakSecp256k sysvar} account.
Moreover, the oracle defines an empty list $A$, which it uses at program runtime to store accounts which public key was compared to $a_{pk}$ (see Line \ref{missing_key_check_line_3}). 

At program runtime, the oracle checks whether the program performs a register comparison operation or a function call operation.
In the case of the register comparison operation, the oracle uses the taint tracking engine to check whether the source and/or destination registers contain account details (see Line \ref{missing_key_check_line_5} and \ref{missing_key_check_line_6}). 
If at least one of the registers contains account details, the oracle checks whether the account details are the public key of an account and whether it is compared with $a_{pk}$ (see Line \ref{missing_key_check_line_7} and \ref{missing_key_check_line_9}). 
If this is the case, the oracle adds the account of the account details to the set $A$ to memorize that the account was compared with $a_{pk}$ before calling the function $f$ (see Line \ref{missing_key_check_line_8} and \ref{missing_key_check_line_10}).

In case the program calls the function $f$ using an eBPF \texttt{CALL} instruction (see Line \ref{missing_key_check_line_11}), the oracle extracts the account $p$ passed to the function (see Line \ref{missing_key_check_line_12}). 
Then the oracle checks if the account $p$ is not included in the set $A$ and thus was not compared with the public key $a_{pk}$ before calling the function $f$ (see Line \ref{missing_key_check_line_13}). 
If this is the case, the oracle signals the VM (see Line \ref{missing_key_check_line_14}).

\begin{algorithm}
\caption{Missing Key Check Oracle}
\label{algorithm:missing_key_check}
\begin{algorithmic}[1]
%\Function{MissingKeyCheckOracle}{}
\State $f \gets \text{function address for which a key check is expected}$                                \label{missing_key_check_line_1}
\State $a_{pk} \gets \text{expected public key to be checked}$                     \label{missing_key_check_line_2}
\State $A \gets \emptyset$                                              \label{missing_key_check_line_3}

\While{program is running}

    \If{program performs register comparison}                           \label{missing_key_check_line_4}
        \State $a \gets \text{account in } src \text{ register}$   \label{missing_key_check_line_5}
        \State $b \gets \text{ account in } dst \text{ register}$   \label{missing_key_check_line_6}
        \If{$a_{pk}$ \textbf{is compared with} $b$.pubkey}        \label{missing_key_check_line_7}
            \State $A \gets A \cup \{b\}$                         \label{missing_key_check_line_8}
        \Else{ $a$.pubkey \textbf{is compared with} $a_{pk}$}     \label{missing_key_check_line_9}
            \State $A \gets A \cup \{a\}$                         \label{missing_key_check_line_10}
        \EndIf
    \EndIf

    \If{program calls function $f$}                                     \label{missing_key_check_line_11}
        \State $p \gets \text{passed account to function } f$                   \label{missing_key_check_line_12}
        \If{$p \notin A$}                                               \label{missing_key_check_line_13}
            \State signal VM                                            \label{missing_key_check_line_14}
        \EndIf
    \EndIf

\EndWhile
%\EndFunction
\end{algorithmic}
\end{algorithm}

\subsection{Integer Bugs Oracle}\label{apx-int}
\Cref{algorithm:integer_bugs} provides a detailed explanation of the \emph{integer bug oracle}.
The oracle operates as follows:
Before the program runs, the oracle initializes an empty list $T$ in which the oracle stores the registers that contain bugged values, i.e., overflowing or underflowing values (see Line \ref{integer_bugs_line_1}). 

At program runtime, the oracle then checks whether an eBPF \texttt{STORE} instruction has caused the program to write a value to a register (see Line \ref{integer_bugs_line_2}). 
If this case occurs, the oracle checks whether the value which the program writes into the register is bugged, i.e. has overflowed or underflowed (see Line \ref{integer_bugs_line_3}).
If a bugged value is written to the register, the oracle remembers the register by adding the register to the list $T$ (see Line \ref{integer_bugs_line_3} and \ref{integer_bugs_line_4}).
In case the program does not write a bugged value to the register, the oracle removes the register from the list $T$ (see Line \ref{integer_bugs_line_5}).

Moreover, the oracle checks if the program writes a value into the lamports field of an account at runtime (see Line \ref{integer_bugs_line_6}).
Then the oracle checks whether the set $T$ contains the register whose value the program writes to the lamports field of an account (see Line \ref{integer_bugs_line_7} and \ref{integer_bugs_line_8}).
This indicates that the program has written a bugged value to the lamports field of the account.
If the program writes a bugged value into the field, the oracle signals the VM (see Line \ref{integer_bugs_line_9}).

\begin{algorithm}
\caption{Integer Bugs Oracle}
\label{algorithm:integer_bugs}
\begin{algorithmic}[1]
%\Function{IntegerBugsOracle}{}
\State $T \gets \emptyset$                                  \label{integer_bugs_line_1}
\While{program is running}
    \If{program writes $value$ to $src$ register}           \label{integer_bugs_line_2}
        \If{$value$ is bugged}                              \label{integer_bugs_line_3}
            \State $T \gets T \cup \{src\}$                 \label{integer_bugs_line_4}
        \Else
            \State $T \gets T \backslash \{src\}$           \label{integer_bugs_line_5}
        \EndIf    
    \EndIf
    
    \If{program writes $value$ to lamports field}           \label{integer_bugs_line_6}
        \State $src \gets \text{register holding } value$   \label{integer_bugs_line_7}
        \If{$src \in T$}                                    \label{integer_bugs_line_8}
            \State signal VM                              \label{integer_bugs_line_9}
        \EndIf
    \EndIf
\EndWhile
%\EndFunction
\end{algorithmic}
\end{algorithm}
